Fully Automated Task Management for Generation, Execution, and Evaluation: A Framework for Fetch-and-Carry Tasks with Natural Language Instructions in Continuous Space

This paper aims to develop a framework that enables a robot to execute tasks based on visual information, in response to natural language instructions for Fetch-and-Carry with Object Grounding (FCOG) tasks. Although there have been many frameworks, they usually rely on manually given instruction sentences. Therefore, evaluations have only been conducted with fixed tasks. Furthermore, many multimodal language understanding models for the benchmarks only consider discrete actions. To address the limitations, we propose a framework for the full automation of the generation, execution, and evaluation of FCOG tasks. In addition, we introduce an approach to solving the FCOG tasks by dividing them into four distinct subtasks.

==> pages/section_4.tex <==
\section{Experimental Setup}

In this study, we newly built the WRS-FC dataset for the FCOG task. The XXXX dataset is a simulation-based dataset consisting of images and natural language instructions. The images were collected by a DSR in the standard simulator used in the World Robot Summit 2018 Partner Robot Challenge/Virtual Space Competition (WRS-VS, [Okada+, AR19]). Each image contains approximately five everyday objects in a room.

We used an extended version of the standard simulator used in WRS-VS. This simulator has a continuous action space, so the robot is capable of executing continuous actions.
